A Review of Machine Learning for Cavitation Intensity Recognition in Complex Industrial Systems

Cavitation intensity recognition (CIR) is a critical technology for detecting and evaluating cavitation phenomena in hydraulic machinery, with significant implications for operational safety, performance optimization, and maintenance cost reduction in complex industrial systems. Despite substantial research progress, a comprehensive review that systematically traces the development trajectory and provides explicit guidance for future research is still lacking. To bridge this gap, this paper presents a thorough review and analysis of hundreds of publications on intelligent CIR across various types of mechanical equipment from 2002 to 2025, summarizing its technological evolution and offering insights for future development. The early stages are dominated by traditional machine learning approaches that relied on manually engineered features under the guidance of domain expert knowledge. The advent of deep learning has driven the development of end-to-end models capable of automatically extracting features from multi-source signals, thereby significantly improving recognition performance and robustness. Recently, physical informed diagnostic models have been proposed to embed domain knowledge into deep learning models, which can enhance interpretability and cross-condition generalization. In the future, transfer learning, multi-modal fusion, lightweight network architectures, and the deployment of industrial agents are expected to propel CIR technology into a new stage, addressing challenges in multi-source data acquisition, standardized evaluation, and industrial implementation. The paper aims to systematically outline the evolution of CIR technology and highlight the emerging trend of integrating deep learning with physical knowledge. This provides a significant reference for researchers and practitioners in the field of intelligent cavitation diagnosis in complex industrial systems.

==> input_figs/input_1_introduction.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth,height=200mm]{figs/Introduction.pdf}
    \caption{Development path and significant milestones of cavitation intensity recognition using machine learning.}
    \label{fig: Introduction}
\end{figure*}

==> input_figs/input_2_ANN.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth,height=70mm]{figs/ANN.pdf}
    \caption{Schematic diagram of a ANN with two hidden layers.}
    \label{fig: ANN}
\end{figure}

==> input_figs/input_2_DT.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth,height=40mm]{figs/DT.pdf}
    \caption{Schematic diagram of a DT. In general, the root node represents the entire sample set.}
    \label{fig: DT}
\end{figure}

==> input_figs/input_2_ES.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth,height=55mm]{figs/ES.pdf}
    \caption{Schematic diagram of an ES.}
    \label{fig: ES}
\end{figure}

==> input_figs/input_2_KNN.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth,height=50mm]{figs/KNN.pdf}
    \caption{Illustration of a KNN algorithm.}
    \label{fig: KNN}
\end{figure}

==> input_figs/input_2_SVM.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth,height=60mm]{figs/SVM.pdf}
    \caption{Schematic diagram of a SVM. The red solid line and the gray dashed line represent the separating hyperplane and the margin boundaries, respectively.}
    \label{fig: SVM}
\end{figure}

==> input_figs/input_2_TML.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth,height=80mm]{figs/TML.pdf}
    \caption{Diagnosis procedure of cavitation intensity recognition using traditional machine learning methods, which consists of data acquisition, feature extraction, feature selection and intelligent intensity recognition.}
    \label{fig: TML}
\end{figure*}

==> input_figs/input_3_Conv.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth,height=60mm]{figs/Conv.pdf}
    \caption{Schematic diagram of convolution operation. (a) and (b) show the working principle of 1D and 2D convolution, respectively.}
    \label{fig: Conv}
\end{figure*}

==> input_figs/input_3_DBN.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth,height=55mm]{figs/DBN.pdf}
    \caption{Schematic diagram of a DBN.}
    \label{fig: DBN}
\end{figure}

==> input_figs/input_3_DL.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.85\textwidth,height=80mm]{figs/DL.pdf}
    \caption{Diagnosis procedure of cavitation intensity recognition using deep learning methods, which consists of data acquisition and data-driven deep learning intensity recognition.}
    \label{fig: DL}
\end{figure*}

==> input_figs/input_3_RNN.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth,height=35mm]{figs/RNN.pdf}
    \caption{Schematic diagram of a RNN.}
    \label{fig: RNN}
\end{figure}

==> input_figs/input_3_Transformer.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth,height=100mm]{figs/Transformer.pdf}
    \caption{Schematic diagram of a Transformer.}
    \label{fig: Transformer}
\end{figure}

==> input_figs/input_4_DKDL.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth,height=70mm]{figs/DKDL.pdf}
    \caption{Diagnosis procedure of cavitation intensity recognition using data and knowledge driven deep learning methods, which consists of data acquisition, knowledge collection, deep feature learning and physical knowledge learning.}
    \label{fig: DKDL}
\end{figure*}

==> input_figs/input_4_PKCL.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth,height=55mm]{figs/PKCL.pdf}
    \caption{Schematic diagram of a PKCL.}
    \label{fig: PKCL}
\end{figure}

==> input_figs/input_4_PKE.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth,height=55mm]{figs/PKE.pdf}
    \caption{Schematic diagram of a PKE.}
    \label{fig: PKE}
\end{figure}

==> input_figs/input_4_PKN.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth,height=65mm]{figs/PKN.pdf}
    \caption{Schematic diagram of a PKN with two physical mechanism hidden layers.}
    \label{fig: PKN}
\end{figure}

==> input_figs/input_5_Discussion.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth,height=190mm]{figs/Discussion.pdf}
    \caption{A roadmap outlining the application of machine learning to intelligent cavitation intensity recognition.}
    \label{fig: Discussions}
\end{figure*}

==> tabs/2_1DataAcquisition.tex <==
\begin{table*}[htbp]
\centering
\footnotesize
\caption{Comparison of different sensors in data acquisition stage of cavitation intensity recognition.}
\label{tab: TML_DataAcquisition}
\setlength{\tabcolsep}{0.4mm}{
\begin{tabular}{c|c|c}
\toprule 
Type              & Principle               & Characteristics                                                  \\ 
\midrule
Ultrasonic Sensor & Analyzes variations in high-frequency               & High resolution, sensitive to medium                             \\
High-speed Camera & Captures bubble flashing frequency                                & High temporal resolution, requires transparent medium, high cost \\
Energy Sensor     & Measurement of energy changes   & Quantitative, requires high-precision devices, high cost         \\
Pressure Sensor   & Detects local pressure pulsations            & High sensitivity, real-time, vulnerable to corrosion and impact  \\
Vibration Sensor  & Monitors surface micro-vibrations           & Flexible installation, low cost, source interference possible    \\
Acoustic Sensor   & Monitors sound wave changes            & Remote monitoring, strong penetration, needs noise suppression   \\ 
\bottomrule
\end{tabular}}
\end{table*}

==> tabs/2_2SVMMethods.tex <==
\begin{table*}[htbp]
\footnotesize
\centering
\caption{Summary of applications of SVM-based methods in cavitation intensity recognition.}
\label{tab: SVM Methods}
\setlength{\tabcolsep}{5mm}{
\begin{tabular}{llc}
\toprule 
Objects & References & Signals \\ 
\midrule
\multirow{4}{*}{Pump} 
            &  \cite{hasanpour2024pump}, 
               \cite{zhou2024multi},
               \cite{shervani2018cavitation},
               \cite{panda2018prediction},
               \cite{li2024intelligent}, 
               \cite{han2024off}, 
               \cite{he2022intelligent},
               \cite{dutta2020comparative},          
               \cite{rapur2019multifault},
               \cite{casoli2019multi},
               & \multirow{4}{*}{Vibration, Pressure, Current, Acoustic} \\
               &
               \cite{qiu2019experimental},
               \cite{tingfeng2011ls},
               \cite{stephen2025evaluation},
               \cite{hu2025cavitation}, 
               \cite{ranawat2025blockage}, 
               \cite{dias2025edge},
               \cite{araste2023fault},
               \cite{huang2023condition},
               \cite{xiao2022research},
               \cite{al4615504incipient},
               &                         \\
               
              & 
               \cite{kamiel2022cavitation},
               \cite{bordoloi2017identification}, 
               \cite{dutta2023svm},
               \cite{araste2020support},
               \cite{youlin2017wavelet},
               \cite{xue2014intelligent},
               \cite{wang2019hydraulic},
               \cite{muralidharan2014fault},
               \cite{sakthivel2010application},
               
               &                         \\

                & \cite{matloobi2018identification}, 
                \cite{al2021faults},
                \cite{altobi2019fault},
                \cite{orru2020machine},
                \cite{song2024centrifugal}
                 &                         \\
               



             
Turbine      & \cite{stephen2025evaluation},
               \cite{gregg2018method},
               \cite{de2019intelligent},
               \cite{liu2014underwater},
               \cite{kang2022cavitation}
             & Vibration, Acoustic         \\ 
             
Pipe         & \cite{de2015cavitation},
               \cite{chen2022csa},
               \cite{bagherzadeh2025prediction},
               \cite{liu2025machine},
               \cite{hong2025improving},
               \cite{dias2024soft}
             & Ultrasonic, Pressure, Acoustic       \\ 
             
Propeller    & \cite{jeong2012surface},
               \cite{gypa2023propeller}
             & Vibration         \\ 


\bottomrule
\end{tabular}}
\end{table*}



==> tabs/2_3DTMethods.tex <==
\begin{table*}[htbp]
\footnotesize
\centering
\caption{Summary of applications of DT-based methods in cavitation intensity recognition.}
\label{tab: DT Methods}
\setlength{\tabcolsep}{5mm}{
\begin{tabular}{llc}
\toprule 
Objects & References & Signals \\ 
\midrule
\multirow{2}{*}{Pump} 
                &  \cite{dutta2018centrifugal},
                   \cite{han2024off},
                   \cite{casoli2019multi},
                   \cite{chang2024random},
                   \cite{kamali2025characterization},
                   \cite{zhang2022anti},
                   \cite{gatica2025classifying},
                   \cite{orhan2024machine},
                   
                   
                & \multirow{2}{*}{Vibration, Current, Acoustic, Ultrasonic, Pressure} \\
                & \cite{karagiovanidis2023early},
                \cite{sakthivel2010vibration}, 
                \cite{muralidharan2013feature},
                  \cite{farokhzad2013fault},
                  \cite{sakthivel2011use},
                  \cite{stephen2024prediction},
                  \cite{manikandan2023vibration}          &                         \\

             
Turbine      & \cite{de2019intelligent},
               \cite{kang2020stacked},
               \cite{gruberdetection},
               \cite{gruber2014detection},
               \cite{kang2022analysis},
               \cite{amihai2018industrial},
               \cite{saari2018selection}

             &  Acoustic, Vibration, Pressure, Ultrasonic  \\ 
             
Pipe         & \cite{sha2022acoustic},
               \cite{liu2025machine},
               \cite{xu2022leakage},
               \cite{shen2022tree}
             & Acoustic, Vibration    \\ 
             
Valve        & \cite{sha2022acoustic},
              \cite{ehemann2023ai},
              \cite{yakupov2023application}
             & Acoustic, Vibration     \\ 


\bottomrule
\end{tabular}}
\end{table*}

==> tabs/2_4ANNMethods.tex <==
\begin{table*}[htbp]
\footnotesize
\centering
\caption{Summary of applications of ANN-based methods in cavitation intensity recognition.}
\label{tab: ANN Methods}
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{llc}
\toprule 
Objects & References & Signals \\ 
\midrule
\multirow{4}{*}{Pump} 
                & \cite{kumar2021identification},
                  \cite{liu2024cavitation},
                  \cite{dong2019cavitation},
                  \cite{casoli2019multi},
                  \cite{stephen2025evaluation},
                  \cite{matloobi2018identification},
                  \cite{al2021faults},
                  \cite{altobi2019fault},
                  \cite{orru2020machine},
                  \cite{song2024centrifugal},
                  
                  
                  
                  
                  
                & \multirow{4}{*}{Current, Pressure, Vibration, Acoustic, High-speed images} \\
                & \cite{de2019intelligent},
                \cite{lavretsky2002health},
                 \cite{bernardini2009expert},
                  \cite{rathinasabapathydevelopment},
                  \cite{kane2016application},
                  \cite{hussain2016condition},
                  \cite{babikir2019noise},
                  \cite{maradey2020methodology},
                  \cite{sayed2020classification},
                  
                  
                  
                
                &  \\

                & 
                \cite{adeodu2020adaptive},
                  \cite{matloobi2021identification},
                  \cite{lan2022experimental},
                  \cite{tong2023cavitation},
                  \cite{nasiri2011vibration},
                  \cite{siano2018diagnostic},
                  \cite{farokhzad2012897},
                  \cite{zhang2016effect},
                  \cite{al2022using},
                  
                  
                  
                &  \\

                & 
                
                  \cite{zouari2004fault},
                  \cite{tan2023fault},
                  \cite{wang2025optimization},
                  \cite{azizi2017improving},
                  \cite{arendra2020investigating},
                  \cite{xu2021multi}
                &  \\

             
Turbine      & \cite{stephen2025evaluation},
               \cite{hovcevar2005prediction},
               \cite{saeed20133d},
               \cite{zhao2020use},
               \cite{souza2024application},
               \cite{de2012neural},
               \cite{sun2019prediction},
               \cite{benabdesselam2025multi}

             & Vibration, Pressure, Ultrasonic, High-speed images  \\ 
             
Pipe         & \cite{de2015cavitation},
               \cite{yang2008leak},
               \cite{wu2023neural},
               \cite{you2024cavitation}
             & Acoustic, Pressure    \\ 
             
Valve        & \cite{salah2019automated},
               \cite{gao2019cavitation}
             & Acoustic, Vibration     \\ 

Propeller    & \cite{schizas2002artificial}
             & Vibration     \\ 


\bottomrule
\end{tabular}}
\end{table*}

==> tabs/2_5CNNMethods.tex <==
\begin{table*}[htbp]
\footnotesize
\centering
\caption{Summary of applications of CNN-based methods in cavitation intensity recognition.}
\label{tab: CNN Methods}
\setlength{\tabcolsep}{5mm}{
\begin{tabular}{lclc}
\toprule 
Objects                  & Types                                       & References & Signals                 \\ 
\midrule
\multirow{7}{*}{pump}    
& \multirow{3}{*}{1D CNN}                     & \cite{tong2023cavitation},
                                                \cite{chao2020cavitation},
                                                \cite{liu2021convolution},
                                                \cite{tiwari2021blockage},
                                                \cite{han2022comparative},
                                                \cite{li2022application},
                                                \cite{han2025use},
                                                \cite{song2025cavitation},
                                                \cite{lu2024research},
                                                
                                                
                                                & \multirow{8}{*}{\makecell{Acoustic, \\Vibration, \\ Pressure,\\ Current, \\ High-speed images}} \\


                                                
&                                             & 
                                                \cite{he2024status},
                                                \cite{turunen2023deep},
                                                \cite{wang2025cavitation},
                                                 
                                                \cite{feng2024experimental},
                                                \cite{vasiliev2023pump},
                                                \cite{pan2018improved},
                                                \cite{zheng2025intensity},
                                                \cite{e2024development},
                                                \cite{ugli2023automatic},
                                                
                                                
                                                &                         \\
                                            && 
                                                
                                                \cite{li2020adaptive},
                                               \cite{zheng2023hydrodynamic},
                                               \cite{guo2022fault}
                                               
                                            
                                            \\
\cmidrule{2-3}
& \multirow{4}{*}{2D CNN}                     & 
                                                \cite{kumar2020improved}, 
                                                \cite{chao2020identification},
                                                \cite{Wei2021cavitation},
                                                \cite{zhu2021intelligent},
                                                \cite{hajnayeb2021cavitation},
                                                \cite{chao2022improving},
                                                \cite{liu2023intelligent},
                                                \cite{chennai2023deep},
                                                \cite{tang2024light},
                                                
                                                
                                                
                                              &                         \\
&                                             & 
                                                \cite{zhu2023data},
                                                \cite{ullah2023intelligent},
                                                \cite{tang2022adaptive},
                                                \cite{prasshanth2024deep},
                                                \cite{prasshanth2024fault},
                                                \cite{chao2023cavitation},
                                                \cite{sun2025cavitation},
                                                \cite{lee2025deep},
                                                \cite{chang2022centrifugal},
                                                
                                                
                                                &                         \\
                                                && 
                                                   \cite{huh2020new},
                                                   \cite{li2024fault},
                                                   \cite{chao2022fault},
                                                   \cite{tang2020intelligent},
                                                   \cite{zaman2023centrifugal},
                                                   \cite{kumar2025inceptionv3},
                                                   \cite{sunal2024centrifugal},
                                                   \cite{ma2023systematic},
                                                   \cite{anvar2023novel},
                                                
                                                \\
                                                && 
                                                  \cite{wang2019novel},
                                                  \cite{dai2023cavitation},
                                                  \cite{li2024vmd}
                                                   
                                                
                                                \\
\midrule


\multirow{3}{*}{Turbine}    
& \multirow{2}{*}{1D CNN}                     & \cite{zheng2025intensity},
                                                \cite{zheng2023hydrodynamic},
                                                \cite{liu2025data},
                                                \cite{singh2025hybrid},
                                                \cite{dao2024wear},
                                                \cite{qian2022cnn},
                                                \cite{chen2025fault},
                                                \cite{jin2019eemd},
                                                \cite{wan2025fault},
                                                
                                        

                                                & \multirow{3}{*}{\makecell{Acoustic, Vibration, \\Pressure, Current}} \\
&                                             & \cite{lin2023application}          &                         \\
\cmidrule{2-3}
& \multirow{1}{*}{2D CNN}                     & \cite{kirschner2023cavitation},
                                                \cite{look2018building},
                                                \cite{tang2022intelligent},
                                                \cite{he2023sgst},
                                                \cite{wang2021high},
                                                \cite{liu2021method},
                                                \cite{xu2023cost}
                                                

&                         \\

\midrule   


\multirow{2}{*}{Pipe}    
& \multirow{1}{*}{1D CNN}                     & \cite{you2024cavitation},
                                                \cite{sha2022regional},
                                                \cite{sha2022multi},
                                                \cite{gou2024hierarchical},
                                                \cite{wang2022deeppipe},
                                                \cite{li2022rolling}

                                                                               & \multirow{2}{*}{Acoustic} \\

\cmidrule{2-3}
& \multirow{1}{*}{2D CNN}                     & \cite{sandhu2024comparative},
                                                \cite{sha2024hierarchical},
                                                \cite{liu2022automatic}
                                              &                         \\

\midrule  

\multirow{2}{*}{Propeller}    
& \multirow{1}{*}{1D CNN}                     & \cite{tsai2021multi},
                                                \cite{jamal2024passive},
                                                \cite{kim2022study}

                                                                                     & \multirow{2}{*}{\makecell{Acoustic, Current, \\High-speed images}} \\

\cmidrule{2-3}
& \multirow{1}{*}{2D CNN}                     & \cite{miglianti2020predicting},
                                                \cite{bach2021classification},
                                                \cite{bach2021enhancing},
                                                \cite{liu2025feature},
                                                \cite{yilmaz2025deep},
                                                \cite{chen2024ship},
                                                \cite{shen2022quantitative},
                                                \cite{sheikh2025marine},
                                                \cite{sheikh2025ensemble}
                                                
                                                &                         \\


\midrule  
\multirow{2}{*}{Valve}    
& \multirow{1}{*}{1D CNN}                     & \cite{sha2022regional},
                                                \cite{sha2022multi},
                                                \cite{gou2024hierarchical}     
                                                
                                                                                     & \multirow{2}{*}{\makecell{Acoustic, \\Vibration}} \\

\cmidrule{2-3}
& \multirow{1}{*}{2D CNN}                     &  \cite{sha2024hierarchical},
                                                \cite{wei2023cavitation}
                                               
                                                    &                         \\


\bottomrule
\end{tabular}}
\end{table*}
